Efficient Deployment of Large Language Models on Resource-constrained Devices

Deploying Large Language Models (LLMs) on resource-constrained (or weak) devices presents significant challenges due to limited resources and heterogeneous data distribution. To address the data concern, it is necessary to fine-tune LLMs using on-device private data for various downstream tasks. While Federated Learning (FL) offers a promising privacy-preserving solution, existing fine-tuning methods retain the original LLM size, leaving issues of high inference latency and excessive memory demands unresolved. Hence, we design FedSpine, an FL framework that combines Parameter- Efficient Fine-Tuning (PEFT) with structured pruning for efficient deployment of LLMs on resource-constrained devices. Specifically, FedSpine introduces an iterative process to prune and tune the parameters of LLMs. To mitigate the impact of device heterogeneity, an online Multi-Armed Bandit (MAB) algorithm is employed to adaptively determine different pruning ratios and LoRA ranks for heterogeneous devices without any prior knowledge of their computing and communication capabilities. As a result, FedSpine maintains higher inference accuracy while improving fine-tuning efficiency. Experimental results conducted on a physical platform with 80 devices demonstrate that FedSpine can speed up fine-tuning by 1.4$\times$-6.9$\times$ and improve final accuracy by 0.4%-4.5% under the same sparsity level compared to other baselines.

==> contents/implemenetation.tex <==
% We have implemented \method with about 3k lines of code using FedScale \cite{lai2022fedscale}, an open-source evaluation platform for federated learning.
% FedSpine adopts a server-device architecture tailored for efficient LLM deployment on resource-constrained devices.
% At the server side, the developer first submits the FL job with the specific criteria for model size to the \textit{Configuration Updater}. 
% \textcircled{2}: Along with the devices’ feedback (\ie, state information) from the last fine-tuning round, the \textit{Configuration Updater} dynamically determine refining configurations (\eg, pruning ratios and LoRA ranks) based on device capabilities. \textcircled{3}: the \textit{Device Distributor} retrieves the participant list and information as well as the most recent global model, which can be transmitted to the Receiver at the corresponding devices.
% \textcircled{4}: Using LoRA gradients from the previous round, the \textit{Model Pruner} performs loss-aware structured pruning to remove low-impact parameters of local LLMs. \textcircled{5}: Given the device’s local data, computational and communication resources, the \textit{Model Fine-Tuner} launches its local fine-tuning process to recover performance with adaptive LoRA ranks. \textcircled{6}: a \textit{resource monitor} to track computation and communication metrics. \textcircled{7}: Finally, the \textit{LoRA Aggregator} collects the updated LoRA weights from all devices and adopts heterogeneity-aware weighted aggregation to update the global model.  
% The iterative process continues until on-device LLMs reaches the target pruning ratio.





 % a fine-tuning module that integrates received LoRA weights with local LLMs for adaptive training on device-specific data , and 



% \method provides streamlined APIs to abstract the complexities of adaptive model pruning and fine-tuning for LLMs. 
% Developers can import \method in their application codebase and interact with FL engines (\eg, PySyft\footnote{https://github.com/OpenMined/PySyft}).
% % or TensorFlow Federated\footnote{https://www.tensorflow.org/federated}).
% \method has been integrated with PySyft, where it operates by managing and continuously updating its device metadata, such as device capabilities. 
% The metadata is cached in memory to support rapid access during execution and is periodically backed up to persistent storage for fault tolerance. 
% In case of system interruptions, the execution driver will initialize a new instance and load the latest checkpoint to resume operations seamlessly.
% For seamless integration with FL engines, \method allows the server to direct model updates and tasks to all devices using PySyft's API. 
% \rednote{Specifically, \textit{model.send(device\_id)} is used to dispatch training tasks based on FedSpine’s refining configurations, and \textit{model.get(device\_id)} retrieves device feedback to further parameter updating.}



% Write a system design with clear logic and fluent sentences






==> contents/intro_bp_1103.tex <==


% To address the issue of resource constraints, Parameter-Efficient Fine-Tuning (PEFT) methods, \eg, Adapter \cite{}, LoRA \cite{}, have been deployed to FL.
% These techniques freeze most LLM parameters and only update a few additional parameters or a part of the original model parameters, thus efficiently reducing LLMs fine-tuning memory and computing consumption.
% However, PEFT models do not improve inference efficiency because the LLM size remains the same or even increases.
% Simultaneously, not all parameters of large models are valid for downstream tasks and redundant parameters could be pruned to reduce model size without sacrificing accuracy performance.
% On the other hand, structured pruning improves inference efficiency by removing grouped parameters such as attention heads and feed-forward neurons, while sparse unstructured pruning models are hard to obtain direct inference speedup without modification to the network structure.

% Existing works mainly focus on integrating structured pruning and PEFT on center server. \cite{} combines PEFT and structured pruning and applies it over LoRA-tuned models, leading to substantial performance loss and extra training costs.

% However, training pruned LMs causes LLMs performance degradation for downstream tasks and takes extra time to converge.
% Moreover, due to system heterogeneity, fast workers may be forced to wait for slow ones, leading to increased waiting time and non-negligible training costs.


% 1.LLM火热背景 .

% 2.大模型压缩的必要性（范围收缩到结构化剪枝）

% 3.现有的剪枝（都是中心化的）：先微调，再剪枝（）<先剪枝，再微调（）<边LORA微调，边剪枝（）
% 4.为了充分利用端侧数据，提出联邦边LORA微调，边微调边剪枝框架。
% 5.这个框架面临两个异构挑战（数据异构和系统异构）。根据数据分布来适应性进行对LLM进行剪枝， 不同的剪枝比会导致效率低下，通过适应性微调来解决系统异构
% 6.介绍我们的技术细节与优点（剪枝技术，微调技术，蒸馏技术 ），突出contribution
\
% in this regard, memory footprint
% start from some killer applications requiring the deployment of LLMs at the network edge.

% Large Language Models (LLMs) \cite{openai2023gpt, touvron2023llama, devlin2018bert, liu2019roberta} have demonstrated exceptional performance in a multitude of natural language processing (NLP) benchmarks (\eg, GLUE, \cite{radford2019language}).
% To further refine these models for a more precise alignment with specific tasks and user preferences, they are often typically fine-tuned on downstream datasets.
% % However, notwithstanding their considerable potential,
% While increasing the scale of LLMs significantly enhances their abilities \cite{kaplan2020scaling}, direct fine-tuning of them incurs substantial computational and memory overhead due to the enormous parameters encompassed. 

%先说明大模型目前比较火热。然后说明终端设备算力的不断提升，Apple、微软等厂商不断推出了能够在终端设备上运行的LLM-driven的AI应用，如Apple Intelligence、Copilot等。通过利用终端上的丰富数据来微调预训练的LLMs可以让LLMs更好地xxxx。
% Large Language Models (LLMs) \cite{openai2023gpt, touvron2023llama, devlin2018bert, liu2019roberta} have demonstrated exceptional performance in a multitude of natural language processing (NLP) benchmarks (\eg, GLUE \cite{radford2019language}).

% The recent advent of Large Language Models (LLMs), such as OpenGPT and LLaMa, marks a substantial breakthrough in Artificial Intelligence (AI) \cite{cao2023comprehensive}. 
% As computing power on end devices continues to grow, tech giants like Apple and Microsoft have launched LLM-driven AI applications, such as Apple Intelligence and Copilot, which are powered by multiple LLMs and designed to accomodate to end devices. 
The recent development of Large Language Models (LLMs), such as OpenGPT and LLaMa, marks a significant milestone in advancing Artificial Intelligence (AI) \cite{cao2023comprehensive}. 
As computational capabilities on end devices continue to improve, leading technology companies, including Apple and Microsoft, have introduced LLM-powered AI applications, such as Apple Intelligence and Microsoft Copilot. 
These applications are driven by multiple LLMs and optimized for deployment on end devices, leveraging local processing to enhance responsiveness and privacy.
% Tech giants, smartphone manufacturers, and chipmakers have launched billion-scale LLMs (\eg, Qwen-1.8B, Phi-2.7B, ChatGLM3-6B, Baichuan2-7B, Gemini-Nano) to continuously provide local service.
% By Leveraging the rich data generated on these end devices, fine-tuning 
However, the heterogeneous and context-specific data generated on end devices often exhibits distributional shifts from the data on which LLMs were pre-trained, necessitating on-device fine-tuning. 
This fine-tuning process helps develop tailored models that better align with the unique requirements of downstream tasks, thereby enhancing task-specific performance and adaptability.


% Considering the state-of-the-art workflow of LLMs, there are three main phases: 1) pre-training LLMs from scratch with extensive computational resources and a large corpus (\eg, Wikipedia).
% 2) fine-tuning pre-trained LLMs for various downstream tasks, and 3) deploying the fined-tuned LLMs on end devices (\eg, smartphones) for inference.
% \rednote{This fine-tuning of LLMs traditionally requires access to vast amounts of data, often sourced from distributed end devices.}
% LLMs are fine-tuned 

However, with the rising privacy concerns, the data protection and privacy regulations like GDPR \cite{voigt2017eu} have limited the collection and sharing of personal raw data.
Thus, it becomes much difficult for a centralized server to collect the data distributed across end devices for LLM fine-tuning. 
To break this barrier, Federated learning (FL) has emerged as a privacy-preserving technique that coordinates end devices to collaboratively train deep learning models without exposing their raw data.
When it comes to LLMs, it is non-trivial to directly deploy LLMs on ``weak'' end devices (with low computing and storage capacities) and conduct full-parameter fine-tuning with FL due to the limited resources of the devices. 
For example, fine-tuning a 13B LLaMA model will cost about 100GB memory footprint, while the end devices are usually equipped with a memory of about 1-8 GB \cite{liao2024parallelsfl}. 
% Meanwhile, it is often impractical for local devices to support full parameter fine-tuning of LLMs because of their limited computing resources. 

To resolve the dilemma, it is appealing to incorporate Parameter-Efficient Fine-Tuning (PEFT) techniques into FL. 
% Recent research efforts have explored
The PEFT methods, such as Adapter \cite{houlsby2019parameter} and LoRA \cite{hu2021lora}, aim to freeze the pre-trained LLM parameters and update only a few additional parameters (typically less than 1\% of the LLM parameters) \cite{zhang2023fedpetuning}, facilitating the implementation of fine-tuning LLMs on resource-constrained end devices with FL.
% These properties reduce computational and memory consumption required by LLMs fine-tuning since end devices just need to tune lightweight parameters for updates.
%这段应该说明为了进一步提升微调效率，我们准备通过模型剪枝来降低微调时大模型前向传播的计算开销。同时这样也有助于提升后期推理的效率。
To further improve fine-tuning efficiency, we aim to reduce the computational overhead of LLM forward propagation during fine-tuning through model pruning \cite{zhu2023survey},  which also enhances the later inference efficiency.
% Nevertheless, \rednote{fine-tuned LLMs still impose substantial resource overhead during inference, as their size remains the same or even increases, limiting their inference efficiency on end devices.}
To mitigate this issue, structured pruning \cite{ma2023llm, kwon2022fast, xia2022structured, zhao2024apt} offers a promising choice by removing grouped parameters, such as attention heads and feed-forward neurons, and has proven more inference speedup than unstructured pruning methods \cite{han2015deep, sanh2020movement}. 

% To mitigate this issue, structured pruning \cite{ma2023llm, kwon2022fast, xia2022structured, zhao2024apt} achieves inference speedup by removing grouped parameters, such as attention heads and feed-forward neurons, and has proven more effective than unstructured pruning methods \cite{han2015deep, sanh2020movement}. 

% The central parameter server (PS) distributes a pre-trained LLM to end devices, and then edge clients perform local
% training using PEFT methods. After training, the central server
% aggregates these updates and redistributes the enhanced LLM
% to edge servers for subsequent training rounds. This iteration continues until the LLM achieves a predefined accuracy threshold.


% , it also incurs significant training and inference costs. 
% For instance, a 13B LLaMA model \cite{} costs about 100GB of memory for fine-tuning
% and 30GB for inference with float16 datatype. 
% Thus, optimizing both training and inference efficiency is essential for deploying LLMs in practical applications.
% 分别引出提高微调和推理效率的办法：peft and 结构化剪枝
% However, deploying a scaled-up LLM onto a resource-constrained end device poses multiple challenges, including inference speed, memory footprint, and resource consumption.

%2. 在终端部署大模型已经成为趋势，说明终端两个特性properties：资源有限、数据分散。从而引出需要微调和剪枝。

% Parameter-efficient fine-tuning (PEFT) methods, such as Adapter \cite{houlsby2019parameter} and LoRA \cite{hu2021lora}, have been explored to reduce computational and memory consumption during fine-tuning. 
% These approaches improve training efficiency by freezing most LLM parameters and updating only a few additional parameters. 
% However, PEFT models do not improve inference efficiency because the LLM size remains the same or even increases.
% In contrast, structured pruning \cite{ma2023llm, kwon2022fast, xia2022structured, zhao2024apt} achieves inference speedup by removing grouped parameters, such as attention heads and feed-forward neurons, and has proven more effective than unstructured pruning methods \cite{han2015deep, sanh2020movement}. 




% Structured pruning offers more inference speedup than sparse unstructured pruning methods \cite{}. 

% Model compression emerges as the silver-bullet solution for reducing deployment costs given an accessible LLM.
% To essentially reduce model computation and memory overhead, pruning aims to discard weights with low salience to the LLM.
% Recently, state-of-the-art (SOTA) unstructured pruning approaches, \ie, SparseGPT \cite{} and Wanda\cite{}, have achieved high-performance unstructured sparse LLMs. 
% However, unstructured sparse models are hard to obtain direct inference speedup or memory saving. They often require specialized hardware support to achieve satisfying acceleration benefits \cite{fang2023depgraph, you2023vitcod}.


% Despite the individual advantages of PEFT and structured pruning, 
While PEFT and structured pruning could be integrated to improve both fine-tuning and inference efficiency, existing research \cite{zhao2023cpet, ma2023llm} indicates that simply combining PEFT and structured pruning leads to substantial performance degradation.
For example, CPET \cite{zhao2023cpet} applies structured pruning over LoRA-tuned models, while LLMPruner \cite{ma2023llm}, a pioneer approach to structured pruning of LLMs, first prunes the model and then uses LoRA fine-tuning for performance recovery. 
However, separation of tuning and pruning in this way can result in sub-optimal results \cite{sanh2020movement, molchanov2019importance}. 
% These issues arise because separating tuning and pruning can lead to sub-optimal results \cite{}.
To address this challenge, APT \cite{zhao2024apt} introduces an adaptive framework that iteratively prunes and tunes LLMs' parameters, yielding significant improvements in both training and inference performance. 
% Nevertheless, the practical deployment of these techniques faces a critical challenge, \ie, privacy concerns.



% In practical scenarios, data distributed across devices are not allowed to be collected to a centralized parameter server (PS) due to privacy concerns, even if they demand a shared LLM with the same downstream task \cite{lin2023pushing}.
% Federated learning (FL) has emerged as a solution that enables collaborative model training without sharing private data. 
% In this context, we propose a novel FL framework, called \method, which combines the benefits of PEFT and structured pruning to improve both fine-tuning and inference efficiency in a privacy-preserving manner. 
% % The system overflow is illustrated in Fig. \ref{}. 
% \method focuses on one of the most prominent PEFT methods, \ie, LoRA \cite{hu2021lora}, which trains low-rank approximations of the original model. 
% The goal of \method is to obtain global LoRA parameters that can be plugged into the LLM for the targeted downstream task across clients. 
% As shown in Figure. \ref{fig: System}, \method not only prunes LLMs parameter on the client but also restores performance by assigning different LoRA ranks based on client capabilities.  
% Therefore, \method could achieve inference speedup with minimal performance degradation. 
% 介绍我们的方法

% However, \method still suffers from two critical challenges in practical applications: 

% 最好开头可以和上一段不要用类似的表述
Despite its potential, applying this approach in federated environments presents two critical challenges. 
its centralized setting is not efficiently adapted to federated environments and causes deterioration in training performance.
Specifically, two critical challenges may be suffered.
1) Statistical Heterogeneity. Since different user preferences and contexts, local data on each device are typically non-independent and identically distributed (Non-IID) \cite{zhao2022fedgan, zhuang2022divergence, yao2024ferrari}. 
Statistical heterogeneity can slow down the convergence rate and even compromise the accuracy of the fine-tuned LLMs \cite{cho2023heterogeneous, zhao2018federated, wang2020optimizing, li2022pyramidfl}.
2) System Heterogeneity. The devices are generally equipped with heterogeneous computing and communication capabilities, which could differ from each other by more than tenfold times \cite{chen2022decentralized, lai2021oort}. 
This discrepancy causes fast devices to wait for slow ones (also known as stragglers), leading to non-negligible waiting time and decreased training efficiency.


% To this end, we propose \method, a novel FL framework that combines the benefits of PEFT and structured pruning to improve both fine-tuning and inference efficiency in a privacy-preserving manner. 

In this paper, we propose \method, a novel FL framework that combines the benefits of PEFT and structured pruning to improve both fine-tuning and inference efficiency in a privacy-preserving manner. 
% The system overflow is illustrated in Fig. \ref{}. 
\method focuses on one of the most prominent PEFT methods, \ie, LoRA \cite{hu2021lora}, which trains low-rank approximations of the original model. 
The goal of \method is to obtain global LoRA parameters that can be plugged into the original LLM for the targeted downstream task across devices and merged into the pruned LLM for the corresponding downstream task on weak devices. 
As shown in Figure. \ref{fig: System}, \method not only prunes LLMs parameter on the device but also restores performance by assigning additional LoRA parameters.  
This allows \method could achieve inference speedup with minimal performance degradation and resource costs. 

\method is crafted to simultaneously tackle the heterogeneity issues through adaptive selects model parameters for pruning and fine-tuning. 
Our approach is based on two key observations. 
First, although LLMs contain general knowledge, the importance of certain parameters varies across different downstream tasks. 
To address it, we propose a novel loss-based prune method and prune redundant LLM parameters that are less relevant to specific fine-tuning tasks, dynamically adjusting pruning ratio based on statistical heterogeneity among devices.
While adaptive pruning could incur extra time to converge, and the gap of training time among devices thus may become larger and the system heterogeneity could be exacerbated.
We mitigate this by adaptively assigning LoRA ranks and pruning ratios to different devices based on device capabilities, adjusting the parameters as needed to reduce the waiting time without sacrificing model performance.
% By continuously adjusting the most suitable parameters (adding more parameters), our approach could improve model performance and overall efficiency. 

% To this end, \method is designed to simultaneously tackle the heterogeneity issues through adaptive selects model parameters for pruning and fine-tuning. 
% Our approach is based on two key observations as follows. 
% First, LLMs contain general knowledge, but the importance of certain parameters varies across different downstream tasks. 
% To address statistical heterogeneity, we prune redundant parameters that are less relevant to specific fine-tuning tasks based on each device's local data distribution.
% Each device prunes different ratios of LLM parameters according to its local data characteristics.
% Adaptive pruning could incur extra time to converge, and the gap of training time among devices thus may become larger and the system heterogeneity could be exacerbated.
% To manage system heterogeneity, we adaptively assign different LoRA ranks for different devices. 
% By continuously adjusting the most suitable parameters (adding more parameters), our approach could improve model performance and overall efficiency. 
% However, due to the setting of different prune ratios, the computing time will be different for each device per round, leading to increased waiting time and decreased training efficiency.
 
In a nutshell, our work makes the following contributions: 
%这里表述的不够准确，特别是第一点，需要结合FL进行说明。
\begin{itemize}
    \item We propose an efficient federated fine-tuning framework for LLMs, termed \method, which addresses both statistical and system heterogeneity through adaptive pruning on LLMs and tuning on LoRA modules. Besides, We theoretically present the convergence analysis for \method by considering structured pruning and LoRA and a theoretical convergence guarantee is provided.
    % To the best of our knowledge, \method is the first federated framework that combines PEFT method and structured pruning, improving both the training and inference efficiency for LLMs. 
    
    % \item \method adaptively prunes and tunes LLM parameters based on the data distribution and system capabilities of devices, effectively 
    \item We adopt a Multi-Armed Bandit (MAB) based online learning algorithm to determine the optimal pruning ratios and LoRA ranks for end devices at each round. The proposed algorithm 
    can significantly reduce the resources overhead during fine-tuning of LLMs while effectively improving the deployment and inference efficiency on weak devices. 
    \item We conduct comprehensive experiments to evaluate the performance of our framework \method. The experimental results show that \method reduces the total training time by xxx\% and achieves xxx$\times$ speed up for inference compared to baselines. 
\end{itemize}

 




==> contents/prelim_bp1115.tex <==
\subsection{Federated Fine-Tuning with LoRA}\label{subsec: federated learning}
Low-rank adaption is one of the dominant methods of PEFT for large pre-trained language models.
In LoRA \cite{hu2021lora}, some pre-trained weights of dense layers of LLMs are summed with parallel linear \rednote{low-rank adapter modules}.
and inserting trainable rank decomposition matrices into each layer of
the pre-trained model.
%这个与LoRA modules指的是同一个东西的话，就尽量不要使用太多不同的称呼。而且这句话感觉没能很好地体现LoRA和原模型之间的关系，而且这句话和后面的句子之间感觉缺少逻辑关系。
LoRA modules are updated during the fine-tuning while the pre-trained weights (denoted as $\mathbf{W}_0 \in \mathbb{R}^{d \times k}$) are kept frozen.
LoRA models the incremental update (denoted as $\Delta \mathbf{W} \in \mathbb{R}^{d \times k} $) of $\mathbf{W}_0$ by representing it using a low-rank decomposition $\Delta \mathbf{W}=$ $\mathbf{B} \mathbf{A}$, where $\mathbf{B} \in \mathbb{R}^{d \times r}$, $\mathbf{A} \in \mathbb{R}^{r \times k}$ are two trainable parameters.
In this way, the output of the current layer $h$ could be represented as:   
\begin{equation} \label{Eq: LoRA}
    h=\mathbf{W}_0 x+\Delta \mathbf{W} x=\mathbf{W}_0 x+\frac{\alpha}{r} \mathbf{B} \mathbf{A} x
\end{equation}
where $\alpha$ is a constant scale hyper-parameter, 
and the rank $r \ll \min (d, k)$ is a hyper-parameter of “intrinsic dimension” that controls the number of trainable parameters.
According to Eq. \ref{Eq: LoRA}, the output from the LoRA module is added \rednote{coordinate-wise} to the output of the original model.

%这短话和前面的一段之间缺少过渡，引出FL显得比较突兀。
\rednote{An FL system usually includes a parameter server} and $N = \{1, 2, \dots, N\}$ devices, which train a global model collaboratively.
When performing LoRA in FL, each device $i \in N $ keeps its local data $\mathcal{D}_n$ and maintains the pre-trained weights and a trainable LoRA weight.
% $\mathbf{W}_0 \in \mathbb{R}^{d \times k}$ 
% $\Delta \mathcal{W} = \{\mathbf{B}, \mathbf{A}\} $.
The optimization task for federated fine-tuning is to collaboratively find the global parameters which we define as $\overline{\mathbf{B}}$ and $\overline{\mathbf{A}}$. 
Given the pre-trained model $\mathbf{W}_0$, the goal of FL is find the optimal model ($\overline{\mathbf{W}} = \mathbf{W}_0 + \overline{\mathbf{B}}$ $ \overline{\mathbf{A}}$) to \rednote{minimize the global loss function}: %下面这个公式没能很好的体现\mathbf{W}_i和\overline{\mathbf{W}}之间的关系是啥？
\begin{equation} \label{Eq: FL}
    \min_{\overline{\mathbf{W}}}{F(\overline{\mathbf{W}})}=\frac{1}{N} \sum_{i=1}^N F_i(\mathbf{W}_i)
\end{equation}
where $ F_i(\mathbf{W}_i) = \frac{1}{| \mathcal{D}_i |  } \sum_{\xi \in \mathcal{D}_i} f(\mathbf{W}_i; \xi)$ is the local loss function of the local model $\mathbf{W}_i$ on device $i$, and $f(\mathbf{W}_i; \xi)$ is the loss over data sample $\xi$ on local dataset $\mathcal{D}_i$.
\rednote{Suppose there are $T$ rounds of fine-tuning in total}. 
In each communication round $t$, the server broadcasts the global LoRA modules replicas $\overline{\mathbf{B}}^{(t)}$, $\overline{\mathbf{A}}^{(t)}$ to the set of $m$ selected devices, denoted as $\mathbf{S}^t$.
Then each selected device $i$ trains the LoRA modules on their local data for a few local iterations (usually with mini-batch SGD), 
% For the mini-batch stochastic gradient descent (SGD) \cite{}, a local iteration can be expressed as follows: 
% \begin{equation}
%     \Delta \hat{\mathbf{W}}_i^h=\Delta \mathbf{W}_i^h-\eta \cdot \nabla F_i\left(\Delta \mathbf{}{W}_i^h\right)
% \end{equation}
and further push the updated models $\overline{\mathbf{B}}^{(t)}$, $\overline{\mathbf{A}}^{(t)}$ to the server for global aggregation.
The server then updates the global LoRA modules and pushes them back to the next set of selected devices for the next training round, \ie, 
\begin{equation}
    \overline{\mathbf{B}}^{(t+1)}=\sum_{i \in \mathcal{S}^{(t)}} \mathbf{B}_i^{(t)} / m, 
\end{equation}

\begin{equation}
    \overline{\mathbf{A}}^{(t+1)}=\sum_{i \in \mathcal{S}^{(t)}} \mathbf{A}_i^{(t)} / m
\end{equation}

==> contents/prelim_bp_1106.tex <==
\subsection{Federated Fine-Tuning with LoRA}\label{subsec: federated learning}
Low-rank adaption is the state-of-the-art method for PEFT of large pre-trained language models.
In LoRA \cite{hu2021lora}, some pre-trained weights of dense layers of  LLMs are summed with parallel linear low-rank adapter modules.
LoRA modules are updated during the fine-tuning while the pre-trained weights (denoted as $\mathbf{W}_0 \in \mathbb{R}^{d \times k}$) are kept frozen.
LoRA models the incremental update of $\mathbf{W}_0$ (denoted as $\Delta \mathbf{W} \in \mathbb{R}^{d \times k} $) by representing it using a low-rank decomposition $\Delta \mathbf{W}=$ $\mathbf{B} \mathbf{A}$, where $\mathbf{B} \in \mathbb{R}^{d \times r}$, $\mathbf{A} \in \mathbb{R}^{r \times k}$ are two trainable parameters.
In this way, the output of the current layer $h$ could be represented as:
\begin{equation} \label{Eq: LoRA}
    h=\mathbf{W}_0 x+\Delta \mathbf{W} x=\mathbf{W}_0 x+\frac{\alpha}{r} \mathbf{B} \mathbf{A} x
\end{equation}
where $\alpha$ is a constant scale hyper-parameter, 
the rank $r \ll \min (d, k)$ is a hyper-parameter of “intrinsic dimension” that controls the number of trainable parameters.
According to Eq. \ref{Eq: LoRA}, the output from the LoRA module is added coordinate-wise to the output of the original model.

An FL system usually includes a parameter server and $N = \{1, 2, \dots, N\}$ devices, which collaboratively train a global model.
Consider LoRA in FL, each device $i \in N $ keeps its local data $\mathcal{D}_n$ and maintains the pre-trained weights and a trainable LoRA weight.
% $\mathbf{W}_0 \in \mathbb{R}^{d \times k}$ 
% $\Delta \mathcal{W} = \{\mathbf{B}, \mathbf{A}\} $.
The optimization task for federated fine-tuning is to collaboratively find the global parameters which we define as $\overline{\mathbf{B}}$ and $\overline{\mathbf{A}}$. 
Given the pre-trained model $\mathbf{W}_0$, the goal of FL is find the optimal model ($\overline{\mathbf{W}} = \mathbf{W}_0 + \overline{\mathbf{B}}$ $ \overline{\mathbf{A}}$) to minimize the global loss function:
\begin{equation} \label{Eq: FL}
    \min_{\overline{\mathbf{W}}}{F(\overline{\mathbf{W}})}=\frac{1}{N} \sum_{i=1}^N F_i(\mathbf{W}_i)
\end{equation}
where $ F_i(\mathbf{W}_i) = \frac{1}{| \mathcal{D}_i |  } \sum_{\xi \in \mathcal{D}_i} f(\mathbf{W}_i; \xi)$ is the local loss function of the local model $\mathbf{W}_i$ on device $i$, and $f(\mathbf{W}_i; \xi)$ is the loss over data sample $\xi$ on local dataset $\mathcal{D}_i$.
Suppose there are $T$ rounds of tuning in total. In each communication round $t$, the server broadcasts the global LoRA modules replicas $\overline{\mathbf{B}}^{(t)}$, $\overline{\mathbf{A}}^{(t)}$ to the set of $m$ selected devices ,denoted as $\mathbf{S}^t$.
Then each selected device $i$ trains the LoRA modules on their local data for a few local iterations (usually with mini-batch SGD), 
% For the mini-batch stochastic gradient descent (SGD) \cite{}, a local iteration can be expressed as follows: 
% \begin{equation}
%     \Delta \hat{\mathbf{W}}_i^h=\Delta \mathbf{W}_i^h-\eta \cdot \nabla F_i\left(\Delta \mathbf{}{W}_i^h\right)
% \end{equation}
and further push the updated model $\overline{\mathbf{B}}^{(t)}$, $\overline{\mathbf{A}}^{(t)}$ to the server for global aggregation.
The server then updates the global LoRA modules and pushes them back to the next set of selected devices for the next training round, \ie,
\begin{equation}
    \overline{\mathbf{B}}^{(t+1)}=\sum_{i \in \mathcal{S}^{(t)}} \mathbf{B}_i^{(t)} / m, 
\end{equation}

\begin{equation}
    \overline{\mathbf{A}}^{(t+1)}=\sum_{i \in \mathcal{S}^{(t)}} \mathbf{A}_i^{(t)} / m
\end{equation}

\begin{figure}[t]
	%	\vspace{-1mm}
	\centering
         % \vspace{-3.5mm}
	\subfigure[Test Accuracy]{
		\centering
		\includegraphics[width=0.455\linewidth]{fig/Test_accuracy.pdf}\label{fig:preliminary_accuracy}
	}
	\subfigure[Average Waiting time]{
		\centering
		\includegraphics[width=0.455\linewidth]{fig/Average_waiting_time.pdf}\label{fig:preliminary_avergae_time}
	}
	\caption{Test accuracy and average waiting time of three approaches.}\label{fig:preliminary}
 \vspace{-1.5mm}
	% \vspace{-3.5mm}
\end{figure}

\subsection{Importance of Adaptive Model Pruning}\label{subsec: model prune}




LLMs have shown remarkable capabilities in language understanding and generation.
However, such impressive capability typically comes with a substantial model size, which presents significant challenges in inference on resource-constrained devices.
To address this challenge, model pruning is proposed to reduce the inference memory and computational cost while achieving almost similar accuracy of the original model \cite{han2015learning, kang2020operation}.
Model pruning approaches can generally be classified into unstructured pruning and structured pruning.
On the one hand, unstructured pruning removes sparse parameters within LLMs, but it requires dedicated hardware support for efficiency gains.
On the other hand, structured pruning \cite{zhao2023cpet, ma2023llm, zhao2024apt, zhang2023loraprune} is designed to remove consistent blocks in transformer layers (\eg, attention heads, FFN neurons, and hidden dimensions). 
Therefore, the resulting model contains fewer parameters and easy to achieve inference speedup without requiring specialized hardware.

Most of the existing model pruning methods are tailored for centralized LLM fine-tuning. 
However, the data in FL is scattered across devices, and the PS does not have access to data for fine-tuning.
Thus these methods \cite{zhao2023cpet, zhao2024apt, ma2023llm,  zhang2023loraprune} cannot be directly applied to the tuning process of FL.
Moreover, arbitrarily applying these structured pruning methods in FL settings can cause performance degradation, as they fail to account for the heterogeneity of devices.

Unlike centralized IID settings, the data distribution of local data among geographically diverse workers varies significantly, which causes statistical heterogeneity and deteriorates the training performance \cite{mcmahan2017communication, zhuang2022divergence}.
To address this issue, \method employs the gradient-guided pruning method to efficiently estimate the importance of pre-trained weights of different devices. 
However, pruning approaches that rely on gradients of the pre-trained weights are not available because LoRA makes them frozen without computing their gradients. 
Therefore, \method employs the gradients of LoRA as an  approximation for the gradients of the pre-trained weights.
In typical fine-tuning, the importance of certain parameters varies across different downstream tasks. 
Pruning LLMs to be identical in size may hinder some models from effectively adapting to their local downstream tasks, which reduces model accuracy.
Besides, uniform pruning can cause weak devices to become the bottlenecks of the model fine-tuning process. 
To this end, we are inspired to design an adaptive FL fine-tuning framework through adaptive model pruning for heterogeneous devices. 
% The idea of adaptive pruning is to remove irrelevant LLM parameter blocks during fine-tuning based on gradients of LoRA. 
Specifically, we adaptively
determine appropriate pruning ratios for heterogeneous devices. 
Given the pruning ratios, devices compute the importance of every batch of data and update the importance of LLMs parameters.
Every few iterations, we remove a portion of important structured weights until the desired sparsity (pruning ratios) is achieved. 

To demonstrate the effectiveness of adaptive LLM pruning in FL, we conduct a set of pre-experiments for fine-tuning the Roberta model on the SST-2 dataset with 10 devices.
We compared two approaches: FedLR, which applies the LoRA fine-tuning technique, and FedLR-AP, which integrates LoRA with adaptive pruning. 
% We record the final test accuracy and average waiting time of models fine-tuned with FedLR and FedAR-AP.
While structured pruning could accelerate inference speed, it often deteriorates the model performance. 
As shown in Figure. \ref{fig:preliminary_accuracy}, the test accuracy of FedLR-AP decrease 1.4\% compared to FedLR.         
Besides, LLM pruning tends to increase convergence time, and varying pruning ratios across devices introduce disparities in training time, thus exacerbating the waiting time. 
Figure. \ref{fig:preliminary_avergae_time} illustrates that FedLR-AP exhibits a longer average waiting time compared to FedLR.

\subsection{Importance of Adaptive Model Tuning}\label{subsec: model prune}
%设备举例
In most PEFT-based FL fine-tuning schemes \cite{zhang2023fedpetuning, yang2024dual, yi2023fedlora}, the devices are assigned identical and fixed LoRA ranks in each round. 
Due to system heterogeneity, fast devices have to wait for slow ones (\ie, stragglers) for global LoRA aggregation.
To evaluate the negative impacts of staggers, we record the completion time of each device for one fine-tuning round in FL.
As shown in Figure. \ref{}, the computing time for fine-tuning and the transmission time of the LoRA modules at each round varies significantly across devices, as the fastest device completes one round x $\times$ faster than the slowest device. 
In other words, about x \% of the fastest device's time is idle and wasted. 


% If the devices are assigned with identical and fixed LoRA ranks, the fast devices are forced to wait for the slow ones, incurring idle waiting time and impairing the fine-tuning efficiency.
To address this, we propose to assign different LoRA ranks to devices with diverse capacities so as to reduce the waiting time and address the system heterogeneity. 
Generally, the devices with higher computing and communication capabilities are configured with larger LoRA ranks, while those with lower capabilities are assigned with small LoRA ranks.
To evaluate the performance of FedLR with adaptive tuning (denoted as FedLR-AT), we measure test accuracy and average waiting time, comparing with the standard FedLR approach. 
As shown in Figures. \ref{fig:preliminary_accuracy} and \ref{fig:preliminary_avergae_time}, with the help of adaptive fine-tuning, FedLR-AT achieves a 0.6\% improvement in test accuracy over FedLR, while simultaneously reducing average per-round waiting time by about xx\%. 
These results demonstrate the effectiveness of FedLR-AT in mitigating system heterogeneity and improving overall fine-tuning performance in FL.
Motivated by the above findings, it is necessary to incorporate pruning and tuning in FL to simultaneously cope with system and statistical heterogeneity. 
% By Figs. \ref{} and \ref{}. SFL \cite{feng2021bafl}


% To illustrate the efficiency of federated fine-tuning with LoRA, we record the average waiting time and completion time of LLM fine-tuning with.
% As shown in Figs. \ref{} and. 


% \subsection{Model Tuning}\label{subsec: model tuning}
 


% We formally define the problem objective as minimizing the task loss $\mathbf{F}$ under
% \subsection{Split Learning}\label{subsec: split}
% To relax the computation burden and train large-scale models on the resource-constrained devices, split learning \cite{gupta2018distributed, vepakomma2018split} is proposed as an alternative solution.
% The core idea of SL is to split the full model $\mathbf{w}$ into two distinct parts 
% $\mathbf{w} = [ \mathbf{w}_{b}, \mathbf{w}_{p} ] $ at the split layer. 
% The first few layers close to the model input form the bottom model $\mathbf{w}_{b}$, while the remaining layers correspond to the top model $\mathbf{w}_{p}$.
% Different from FL, only the bottom model $\mathbf{w}_{b}$ is distributed to the devices, while the top model $\mathbf{w}_{p}$ is processed on the server in SL \cite{vepakomma2018split}.
% As illustrated in Fig. \ref{fig: System}(b), the training process of SL includes two main steps, \ie, forward propagation (FP) and backward propagation (BP).
% Specifically, the client performs FP based on the bottom model $\mathbf{w}_{b}$ with its local data, and sends the smashed data as well as the corresponding labels to the server.
% Subsequently, the server continues to perform FP and BP to update the top model $\mathbf{w}_{p}$, and sends the backpropagated gradients back to the client to complete BP and update the bottom model $\mathbf{w}_{b}$.

% Generally, the bottom model $\mathbf{w}_{b}$ is updated as follows:
% \begin{equation} \label{Eq: bottom model udpate}
%     \mathbf{w}_{b}' = \mathbf{w}_{b} -\eta \nabla F_{b}(\mathbf{w}_{b}),
% \end{equation}
% where $\eta$ is the learning rate, $\nabla F_{b}(\mathbf{w}_{b}) = \frac{1}{| \mathcal{D} |} \sum_{\xi \in \mathcal{D}} \nabla f(\mathbf{w}_{b};\xi)$ is the gradient derived from a certain mini-batch in dataset $\mathcal{D}$, and 
% $\nabla f(\mathbf{w}_{b};\xi)$ denotes the stochastic gradient regarding the bottom model $\mathbf{w}_{b}$ and input data sample $\xi$.
% Upon the smashed data $g_{\mathbf{w}_{b}'}(\xi)$ received from the client, the top model $\mathbf{w}_{p}$ is updated as follows:
% \begin{equation}\label{Eq: top model update}
%     \mathbf{w}_{p}' = \mathbf{w}_{p} - \eta \nabla F_{p}(\mathbf{w}_{p}).
% \end{equation}
% Here, $\nabla F_{p}(\mathbf{w}_{p})= \frac{1}{| \mathcal{D} |}  
% \sum_{\xi \in  \mathcal{D}} \nabla f(g_{\mathbf{w}_{b}'}(\xi);\mathbf{w}_{p})$ is the gradient of the loss function, and $\nabla f(g_{\mathbf{w}_{b}'}(\xi);\mathbf{w}_{p})$ denotes the stochastic gradient regarding the top model $\mathbf{w}_{p}$ and the smashed data.
% Since the client only trains the bottom model, the computation burden on the client can be obviously reduced, compared to FL.


% % To train with a large-scale model in EC system, SL \cite{gupta2018distributed, vepakomma2018split} is proposed as an alternative solution to reduce the computation burden at the clients compared to FL.
% % The core idea of SL methods is to split the full model $\mathbf{w}$ into two distinct parts 
% % $\mathbf{w} = [ \mathbf{w}_{b}, \mathbf{w}_{p} ] $ at the split layer. 
% % The first few layers $\mathbf{w}_{b}$ correspond to the bottom model, and the remaining layers $\mathbf{w}_{p}$ correspond to the top model.
% % %  $\mathbf{w}_{b}$ consists of the first few layers, and 
% % In vanilla SL\cite{vepakomma2018split}, the top model $\mathbf{w}_{p}$ is processed and computed on the PS while only one client is randomly selected from all clients to train the bottom model $\mathbf{w}_{b}$.
% % % where these portions are processed and computed on different clients. 

% % % Assumed that the first sub-model is trained and accessed on client $i$; the second sub-model is trained and accessed by the 
% % % client  $j$. The client $j$ has no access to client $i$' sub-model and data, which provides privacy protection.
% % The workflow of vanilla SL is illustrated in Fig. \ref{fig: SL}. The whole model training involves two main steps, \ie, forward propagation (FP)
% % on the client and PS, and backward propagation (BP) on the PS and client.
% % Firstly, the client performs FP on local data, and sends smashed data as well as the corresponding labels to the PS. 
% % After that, the PS continues and completes the FP/BP to update the top model $\mathbf{w}_{p}$.
% % Subsequently, the PS sends the backpropagated gradients back to the client to update $\mathbf{w}_{b}$ by proceeding BP process.
% % Based on the local loss function, $\mathbf{w}_{b}$ is updated as follows:
% % \begin{equation} \label{Eq: bottom model udpate}
% %     \mathbf{w}_{b}' = \mathbf{w}_{b} -\eta \nabla F_{b}(\mathbf{w}_{b})
% % \end{equation}
% % where $\eta$ is the learning rate, $\nabla F_{b}(\mathbf{w}_{b}) = \frac{1}{| \mathcal{D} |} \sum_{\xi \in \mathcal{D}} \nabla f(\mathbf{w}_{b};\xi)$ is the gradient of $\mathbf{w}_{b}$, and 
% % $\nabla f(\mathbf{w}_{b};\xi)$ denotes the stochastic gradient given $\mathbf{w}_{b}$ and input sample $\xi$. 
% % Based on smashed data $g_{\mathbf{w}_{b}'}(\xi)$ received from $\mathbf{w}_{b}$, $\mathbf{w}_{p}$ is also updated according to
% % \begin{equation}\label{Eq: top model update}
% %     \mathbf{w}_{p}' = \mathbf{w}_{p} - \eta \nabla F_{p}(\mathbf{w}_{p},\mathbf{w}_{b}')
% % \end{equation}
% % Here, $\nabla F_{p}(\mathbf{w}_{p} ,\mathbf{w}_{b}')= \frac{1}{| \mathcal{D} |}  
% % \sum_{\xi \in  \mathcal{D}} \nabla f(g_{\mathbf{w}_{b}'}(\xi);\mathbf{w}_{p})$ is the gradient of
% % $\mathbf{w}_{p}$, and $\nabla f(g_{\mathbf{w}_{b}'}(\xi);\mathbf{w}_{p})$ denotes the stochastic gradient given the top model $\mathbf{w}_{p}$ and smashed data.
% % % Then the client $j$ transmits the backpropagated gradients back to the client $i$ to 
% % % update its bottom model through backward propagation.
% % % performance by parallelizing SL The bottom submodel $\mathbf{w}_{b}$ and top submodel $\mathbf{w}_{p}$ are distributed to different clients for processing local data and completing the forward/backward propagation, respectively.
% % % Take the CNN model as an example, the bottom model primarily comprises the convolutional layers, while the top model consists of the fully-connected layers.
% % Since each client only needs to train the first layers of the  model, the computation burden on each client can be obviously reduced.
% % % However, existing SL-based ideas, \eg, SplitFed \cite{thapa2022splitfed}, might face a few challenges, such as heterogeneous client properties, latency and communication efficiency. 
% % % All participating clients need to receive backpropagated signals from the server to update their models. This process introduces significant
% % %  time delays and requires substantial communication resources at each global round.

% \subsection{FL with Model Splitting and Client Pairing}

% % Combing with SL method and address these challenges,
% Combining the advantages of FL and SL, we propose our FL framework, namely PairingFL, which perform FL with model splitting and client pairing.
% The model splitting operation is similar to that in Section \ref{subsec: split}.
% The difference between SL and PairingFL lies in the training of the top model.
% In PairingFL, both the bottom model and the top model are trained on the clients, and the partial models are transmitted to the PS for global aggregation.
% As for client pairing, it includes the basic operations of client partitioning and client matching as follows.
% % In PairingFL, each pair of paired clients, separately maintaining the bottom model and the top model, jointly completes local updating by exchanging smashed data as well as gradients, and then sends their local models to the PS for combination and aggregation.
% % We illustrate the workflow of split learning, federated learning, and our proposed framework (\ie, PairingFL) in Fig. \ref{fig: System}.
% % Respectively, we divide the client set into two parts in FL, where one of the parts trains with bottom models and the other is responsible for loading the top models.
% % We perform  to obtain paired clients. 
% % The training process of our framework comprises $H$ rounds, and each round consists of the following phases. 
% % Our core design includes performing client partitioning and matching as follows:

% % \textbf{(1) Client Partitioning for Executing Bottom Models.}
% \textbf{Client Partitioning.}
% % The PS splits the full model into two submodels $\mathbf{w}^h = [ \mathbf{w}_{b}^h, \mathbf{w}_{p}^h ] $,
% In round $h$, the PS carefully partitions all clients into two parts (\ie, $\mathcal{M}^h$ and $\mathcal{N} \backslash  \mathcal{M}^h$), where $M=|\mathcal{M}^h|=\lfloor N/2 \rfloor$.
% The client $i \in \mathcal{M}^h$ and the client $j \in \mathcal{N} \backslash  \mathcal{M}^h$ download bottom model $\mathbf{w}_{b,i}^h$ and top model $\mathbf{w}_{p,j}^h$ from the PS, respectively.
% Since only the local data of these clients in $\mathcal{M}^h$ contribute to the current round of training, we need to carefully design the partitioning strategy with the knowledge of all clients' data distributions.
% % each containing $M=\lfloor N/2 \rfloor$ clients, and these clients will be paired one by one.
% % Let $M$ = $\lfloor N/2 \rfloor$ denotes the number of pairs, where $M=N/2-1$ for odd numbers of clients and $M=N/2$ for even numbers of clients.
% % In round $h$, each client $i$ from front part, denoted as $\mathcal{M}^h$, are selected to download bottom model $\mathbf{w}_{b}^h$ and 
% % each remaining client $j \in \mathcal{N} \backslash  \mathcal{M}^h$ download top model $\mathbf{w}_{p}^h$ from the PS, respectively.
% %  a set $\mathcal{M}^h$ consists of $N/2$ clients considering statistical heterogeneity. 
% % We perform client partitioning by analyzing the data distribution of clients in $\mathcal{M}^h$, since only the local data of these clients contribute to the current round of training.
% % Bottom models are executed on these clients, denoted as $\mathcal{M}^h$, where only the local data on the set contributes to the current round of  training. 
% % However, clients located in geographically distinct regions generate data that follow different distributions, resulting in non-IID data.
% However, due to diverse local environments and user preferences, individual clients often possess non-IID data.
% The clients with similar data distribution probably provide similar and redundant gradient information for model updating, which fails to capture the population distribution of all clients' data. 
% Appointing these clients for training bottom models not only leads to resource waste but also incurs bias in the global model, exacerbating the negative impact of non-IID data on training performance.
% To this end, as in \cite{balakrishnan2022diverse}, we introduce diversity for client partitioning and select the representative clients to form $\mathcal{M}^h$ while adhering to resource constraints. 
% The aggregated model updates of the clients in $\mathcal{M}^h$ are expected to closely approximate the logically aggregated updates of all clients. 
% By encouraging diversity in client partitioning, 
% % we will reduce redundant communication and the impact of under-represented clients who contribute distinct information will be amplified.
% PairingFL effectively mitigates the bias caused by data non-IIDness and speeds up the convergence rate.
% In addition, to further promote fairness, we keep track of how frequently each client engages in adopting its local data to train the bottom model, and will assign larger probabilities for being selected in $\mathcal{M}^h$ to the clients with lower frequencies.
% With this consideration, all clients will experience the chance to contribute their local data to train the global model.

% % \textbf{(2) Client Pairing for Loading Top Models.}
% \textbf{Client Matching.}
% After client partitioning, each client $i \in \mathcal{M}^h$ maintaining the bottom model $\mathbf{w}_{b,i}^h$ needs to be matched with a client $j \in \mathcal{N} \backslash  \mathcal{M}^h$ maintaining the top model $\mathbf{w}_{p,j}^h$ together to complete the local training in round $h$.
% In order to improve collaboration, the matched clients are implemented to work in a one-to-one manner. 
% % $i$ and client $j$ that are already paired will not be paired with others.
% Therefore, we can obtain $M$ paired clients, and each pair performs the local training of the full model as one client does in typical FL.
% Obviously, random matching can be regarded as the simplest matching strategy.
% However, due to system heterogeneity, the computing time of the bottom and top models, as well as the communication time of smashed data/backpropagated gradients between each pair, are highly different.
% The random strategy probably leads the fast pairs to wait for the slow pairs, incurring non-negligible waiting time and significantly reducing the training efficiency.
% Accordingly, we need to carefully design the matching strategy in PairingFL after client partitioning.
% Generally, 
% % it is feasible to estimate the computing time of training the bottom or top models on each client, and the communication time between clients according the historical records.
% by estimating the computing time of training the bottom or top model on client $i \in \mathcal{M}^h$ or client $j \in \mathcal{N} \backslash  \mathcal{M}^h$, and the communication time between clients $i$ and $j$, we will obtain the rough local updating time of all possible pairs.
% After that, we can develop a greedy matching strategy that ensures the local updating time of different pairs is approximately equal, so as to reduce waiting time and improve training efficiency.
% More details will be discussed in Section \ref{sec:algorithm}.
% % After partitioning, the remaining client $j \in \mathcal{N} \backslash  \mathcal{M}^h$ perform the training of the top models, and these clients need to be matched with the previous clients one by one to obtain paired clients. 
% % Within each pair, the clients separately maintain the bottom model and the top model, and collaboratively perform local updates to train the full model. 
% % As shown in Fig. \ref{fig: System}, in round $h$, client $j$ will match with client $i$ to form a pair $\{i,j\} (\forall i \in \mathcal{M}^h, j \in \mathcal{N} \backslash  \mathcal{M}^h)$, where a full model is trained by performing multiple local iterations on the pair.  
% % The one-to-one correspondence between them can be represented using a one-to-one mapping, denoted as $\mathcal{M}^h \rightarrow \mathcal{N} \backslash \mathcal{M}^h$. 
% % Due to system heterogeneity, the computing time of the bottom/top model and the communication time of smashed data/backpropagated gradient among pairs are highly different. 
% % Therefore, the total consumption time (including computing and communication time) of each pair 
% % $r ( r \in {1, 2, \cdots, M} )$ is distinct.
% % % Noted the maximum value of $r$ is $N/2-1$ when the number of clients is odd while $N/2$ for $N$ is even. 
% % Fast pair has to wait for slow ones, resulting in notable waiting time and significantly reducing the training efficiency. 
% % Generally, we expect to match client $i$ with client $j$ in order to balance the total time consumption for each pair $r$.
% % After that, the waiting time among pairs would be significantly reduced.

% Since the partitioning strategy and matching strategy are coupled in PairingFL, we need to make a joint optimization of client partitioning and client matching to simultaneously address statistical heterogeneity and system heterogeneity.
% % }



% \subsection{Model Updating in PairingFL}

% % performs forward propagation over its local dataset and sends split layer representations (also known as smashed data) to the matched client $j$.
% % Each client $i \in  \mathcal{M}^h$ performs forward propagation over its local dataset
% %     % predefined $\tau$ iterations 
% % and sends split layer representations (also known as smashed data) to the matched client $j$.
% % Let $\mathbf{w}_{b,i}^{h,k}$ denotes the bottom model at the $k$-th iteration in round $h$. Therefore, one iteration on client $i$ is expressed as follows:
% % \begin{equation}
% %     \mathbf{w}_{b,i}^{h,k+1} = \mathbf{w}_{b,i}^{h,k} -\eta \nabla F_{b,i}(\mathbf{w}_{b,i}^{h,k}; \xi)
% % \end{equation}
% % Here, $\eta_h $ is the learning rate in round $h$, $\nabla F_{b,i}(\mathbf{w}_{b,i}^{h,k};\xi) = \frac{1}{| \mathcal{D}_i |} \sum_{\xi \in \mathcal{D}_i} \nabla f(\mathbf{w}_{b,i}^{h,k};\xi)$ is the gradient of client $i$, and 
% % $\nabla f(\mathbf{w}_{b,i}^{h,k};\xi)$ denotes the stochastic gradient given $\mathbf{w}_{b,i}^{h,k}$ and input sample $\xi$. 
% % After that, the client $j$ continues and completes the forward/backward propagation to update the top model. And also one iteration for top model is formulated as follows:
% % \begin{equation}
% %     \mathbf{w}_{p,j}^{h,k+1} = \mathbf{w}_{p,j}^{h,k} - \eta_h \nabla F_{p,i}(\mathbf{w}_{p,j}^{h,k};\mathbf{w}_{b,i}^{h,k+1})
% % \end{equation}
% % Here, $\nabla F_{p,i}(\mathbf{w}_{p,j}^{h,k} ,\mathbf{w}_{b,i}^{h,k+1})= \frac{1}{| \mathcal{D}_i |}  
% % \sum_{\xi \in  \mathcal{D}_i} \nabla f(g_{\mathbf{w}_{b,i}^{h,k+1}}(\xi);\mathbf{w}_{p,j}^{h,k})$ is the gradient of
% % client $j$, and $\nabla f(g_{\mathbf{w}_{b,i}^{h,k+1}}(\xi);\mathbf{w}_{p,j}^{h,k})$ denotes the stochastic gradient given the top model $\mathbf{w}_{p,j}^{h,k}$ and smashed data from client $i$.
% % Then the client $j$ transmits the backpropagated gradients back to the client $i$ to 
% % update its bottom model through backward propagation. 

% In round $h$, we can get a pair set $R^h$ with totally $M$ client pairs after client pairing. 
% For a certain pair $r=$ ($i$, $j$) $\in R^h$, $\mathbf{w}_{b,i}^{h,k}$ and $\mathbf{w}_{p,j}^{h,k}$ separately denote the bottom model of client $i$ and the top model of client $j$ at iteration $k$ in round $h$.
% Thus, the model updating of one iteration on clients $i$ and $j$ can be expressed as:
% \begin{equation} \label{bottom model udpate}
%     \mathbf{w}_{b,i}^{h,k+1} = \mathbf{w}_{b,i}^{h,k} -\eta \nabla F_{b,i}(\mathbf{w}_{b,i}^{h,k}),
% \end{equation}
% \begin{equation}\label{Eq: top model update}
%     \mathbf{w}_{p,j}^{h,k+1} = \mathbf{w}_{p,j}^{h,k} - \eta \nabla F_{p,j}(\mathbf{w}_{p,j}^{h,k}),
% \end{equation}
% where $\eta$ is the local learning rate.
% After repeating $\tau$ iterations, the PS collects the bottom model $\mathbf{w}_{b,i}^{h,\tau}$ and top model from each pair and splices them to get the full model.
% The PS aggregates the spliced full models from client pairs as follows:
% % $M$ pairs of paired clients are obtained by client partitioning and matching. 
% % As illustrated in Fig. \ref{fig: System}, the paired clients $\{i,j\}$ perform FP/BP on client $i$ and $j$, respectively, to complete one local iteration. Let $\mathbf{w}_{b,i}^{h,k}$ denotes the bottom model of client $i$ at the $k$-th iteration in round $h$. Therefore, one iteration on client $i$ is expressed as follows according to Eq. \eqref{Eq: bottom model udpate}:
% % \begin{equation} \label{bottom model udpate}
% %     \mathbf{w}_{b,i}^{h,k+1} = \mathbf{w}_{b,i}^{h,k} -\eta \nabla F_{b,i}(\mathbf{w}_{b,i}^{h,k})
% % \end{equation}
% % Accordingly, one iteration for the top model $\mathbf{w}_{p,j}^{h,k}$ of client $j$ at the $k$-th iteration in round $h$ is expressed based on Eq. \eqref{Eq: top model update}:
% % \begin{equation}\label{Eq: top model update}
% %     \mathbf{w}_{p,j}^{h,k+1} = \mathbf{w}_{p,j}^{h,k} - \eta \nabla F_{p,j}(\mathbf{w}_{p,j}^{h,k})
% % \end{equation}
% % After repeating $\tau$ iterations for all the pairs, the PS needs to aggregate bottom model $\mathbf{w}_{b,i}^{h,\tau}$ and top model $\mathbf{w}_{p,j}^{h,\tau}$ from different pairs, respectively.
% % %  where are uploaded to the PS for global aggregation.
% % % Upon receiving all model updates from all pairs,
% % The PS first combines the bottom model and top model from pair $r ( \forall r \in {1, 2, \cdots, M })$ into a full model
% % $\mathbf{w}_r^{h} $ and then aggregates them to obtain $\mathbf{w}^{h+1}$ for the next round as follows:
% \begin{equation}\label{Eq: aggregation}
%     \mathbf{w}^{h+1} = \frac{1}{M} \sum_{r=1}^{M}\mathbf{w}_r^{h}.
% \end{equation}
% The computing time of performing one local iteration on clients $i$ and $j$ is separately denoted as $\mu_{b,i}^{h,k}$ and $\mu_{p,j}^{h,k}$, while the corresponding communication time between clients $i$ and $j$ is defined as $\beta_{i,j}^{h,k}$ at iteration $k$ in round $h$.
% % Given that the upload bandwidth is typically lower than the download bandwidth in conventional WANs, we focus on the communication time involved in transmiting the smashed data from client $i$ to client $j$.
% % Besides, the communication time between client $i$ and client $j$ is denoted as $\beta_{i,j}^{h,k}$   
% % at $k$-th iteration on the $h$-th round.
% Therefore, the duration time (including computing time and communication time) of pair $r$ at iteration $k$ in round $h$ is expressed as:
% \begin{equation}
%     t_r^{h,k}=\mu_{b,i}^{h,k} +\mu_{p,j}^{h,k} + \beta_{i,j}^{h,k}.
% \end{equation}
% % For each global round, the PS needs to collect $\mathbf{w}_{b,i}^{h,\tau}$ and $\mathbf{w}_{p,j}^{h,\tau}$ from all clients for aggregation, respectively. 
% We define the transmission time of uploading bottom model $\mathbf{w}_{b,i}^{h,\tau}$ and top model $\mathbf{w}_{p,j}^{h,\tau}$ of clients $i$ and $j$ in round $h$ to the PS as $\beta_i^h$ and $\beta_j^h$, respectively.
% Accordingly, the local updating time of pair $r$ in round $h$ is formulated as follows:
% %  the completion time of aggregation in round $h$ can be expressed as:
% \begin{equation} \label{eq: time for pair}
%     t_r^h=\tau \cdot t_r^{h,k} +  \max\{\beta_i^h, \beta_j^h \}.
% \end{equation}
% % where $\tau$ is the number of local iterations in a round. 
% % \begin{equation}
% %     t^h=\sum_{k=1}^{\tau} t_{[i,j]}^{h,k} + \max\{\beta_i^h, \beta_j^h \} 
% % \end{equation} 
% Subsequently, the waiting time of pair $r$ in round $h$ can be formulated as $t^h-t_r^h$, where $t^h=\max\{t_r^h | \forall  r \in {1, 2, \cdots, M }\}$ denotes the local updating of the slowest pair.
% $t^h$ also denotes the completion time of round $h$.
% Then the average waiting time of all pairs in round $h$  can be formulated as:
% \begin{equation}
%     \mathcal{W}^h =\frac{1}{M}  \sum_{r=1}^{M}(t^h-t_r^h), \forall  r \in {1, 2, \cdots, M }.
% \end{equation}
% PairingFL ensures to minimize the average waiting time to mitigate the negative impacts of the synchronization barrier.



% % Considering the heterogeneity among clients, the local training performed by each client will vary in terms of their consumption of computing and communication resources.
% % We define the the computing resource consumption of one local iteration for client $i$ and client $j$ as $c_i$ and $c_j$, respectively. The communication resource consumption of transmiting
% % bottom model on client $i$ and top model on client $j$ at global round are denoted as $a_i$ and $a_j$, and $b_i$ and $b_j$ denotes the communication resource consumption of uploading smashed data from 
% % client $i$ to client $j$ and delivering backpropagated gradients from client $j$ to client $i$, respectively.
% % Assuming that the total budgets for computing and communication resources are represented as C and B, respectively.
% % the computing and communication resource constraint
% % are formulated as follows:
% % \begin{equation}
% %     \sum_{h=1}^{H}(\sum_{i=1}^{N/2}c_i+\sum_{j=1}^{N/2}c_j) \le C
% % \end{equation}
% % \begin{equation}
% %     \sum_{h=1}^{H}(\sum_{i=1}^{N/2}(b_i+a_i)+\sum_{j=1}^{N/2}(b_j+a_j)) \le B
% % \end{equation}
% \subsection{Problem Formulation}

% Given an FL task in resource-constrained EC systems, we carefully make the partitioning and matching strategies to minimize the training time under the constraints.
% Accordingly, we formulate the problem as follows:
% % our objective is to minimize the training time on the premise of meeting accuracy requirements and the average waiting time limitations. We give the following problem formulation: 

% \vspace{0.1cm}
% \centerline{$\min \sum\limits_{h=1}^{H}t^h $}
% \vspace{-0.1cm}
% \begin{equation}\label{problem}
%     s.t.
%     \begin{cases}
%     F(\mathbf{w}^H)-F(\mathbf{w}^*) \le \epsilon , \\
%     t_r^h=\tau \cdot (\mu_{b,i}^{h,k} +\mu_{p,j}^{h,k} + \beta_{i,j}^{h,k} )+  \max\{\beta_i^h, \beta_j^h \} , \\
%     \mathcal{W}^h =\frac{1}{M}  \sum_{r=1}^{M}(t^h-t_r^h) \le \varepsilon ,\\
%     % \sum_{h=1}^{H}\tau (\sum_{i=1}^{N/2}c_i+\sum_{j=1}^{N/2}c_j) \le C , \\
%     % \sum_{h=1}^{H}  (\sum_{i=1}^{N/2}(\tau b_i+a_i)+\sum_{j=1}^{N/2}(\tau b_j+a_j)) \le B, \\
%     % \forall i \in \mathcal{M}^h \rightarrow \forall j \in \mathcal{N} \backslash \mathcal{M}^h \\ 
%     r= (i,j), \forall r \in {1, 2, \cdots, M. } \\ 
%     % , \quad\quad\ \  \forall h \in  [H]\\
%     \end{cases}
% \end{equation}
% The first inequalities express the convergence requirement, where $\epsilon > 0$ is the convergence threshold of the training loss between
% the optimal $F(\mathbf{w}^*)$ and $F(\mathbf{w}^H)$ after $H$ rounds. The second equalities indicate the local updating time of the pair $r$ in round $h$.
% The third inequalities denote that the average waiting time of all pairs in each global round should not exceed the predefined threshold $\varepsilon > 0$ (close to zero).
% %  The last two inequalities indicate that the accumulated computing and communication resources can not exceed the respective budgets allocated for computing and communication resources after H global rounds.
% Our objective is to minimize the training time while adhering to the resource constraints and performance requirements.


 
